Synthesizing the Born rule with reinforcement learning

According to the subjective Bayesian interpretation of quantum theory (QBism), quantum mechanics is a tool that an agent would be wise to use when making bets about natural phenomena. In particular, the Born rule is understood to be a decision-making norm, an ideal which one should strive to meet even if usually falling short in practice. What is required for an agent to make decisions that conform to quantum mechanics? Here we investigate how a realistic (hence non-ideal) agent might deviate from the Born rule in its decisions. To do so we simulate a simple agent as a reinforcement-learning algorithm that makes `bets' on the outputs of a symmetric informationally-complete measurement (SIC) and adjusts its decisions in order to maximize its expected return. We quantify how far the algorithm's decision-making behavior departs from the ideal form of the Born rule and investigate the limiting factors. We propose an experimental implementation of the scenario using heralded single photons.

==> deleted_comments.tex <==
location: before figure example_runs
%As an example, we run our algorithm for 200 different data sets in a fixed LE, each constructed such that $p=0.22$ and $(1-p)$ are the probabilities of obtaining 1 and 0, respectively, in each step $s$. For convenience, the data dimensions $\mathcal{S}$ is fixed at $3\times10^{5}$. We allow the agent to choose between $N=50$ different  bets. The results are shown in the histogram in Fig. \ref{fig:example_runs}(a). 

location: after figure example_runs
%\begin{figure}
%\includegraphics[width=8cm]{RewardFunctionsVSSteps_probabilities.pdf}
%\caption{ Reward function used for our algorithm to choose the best action. Our agent calculates these values over $N$ steps and returns the action that gives the higher reward (the maximum point in the fig.). In red, we can see the theoretical value for the case of p=0.23, and the other lines represent the values calculated for our agent for different step numbers. } 
%\label{fig:RF}
%\end{figure}

location: discussion about obtaining experimental phi matrix
%It is worth noting that if just the  minimum number of equations to resolve the linear system is utilized, fluctuation \john{(I don't think fluctuation is the reason here, I think it's becuase the linear system is underdetermined until you have at least a spanning set of input states and measurements, so in principle I think one could get away with 16 properly chosen, but 24 is fine here. Matt, do you agree?)} \matt{Yes, that makes sense to me.} \rodrigo{(what we are trying to explain here is that, due to the imprecision of our agent to learn probabilities, use just the minimum set of probabilities will lead us to a wrong solution.)}introduced by our agent will lead to incorrect solution.

analysis:
%we observe that the Gaussian distribution fitting our results is not centered at $TR_e$, as is expected. We also observe that the standard deviation  is $\sigma_{TD}=0.8$, which represent eight percent of the total value, obtaining a large relative error.

after fig trace_simulation
%\gabo{Furthermore, we investigate how our algorithm converges to smaller $\sigma_E$. As we have just observed, the algorithm does not learn the exact value of the probability expected. Instead, it mostly learns  probabilities inside some interval $I_c$. This fluctuations  affects the learning of the $\Phi$ matrix.\sout{ In this case, the reconstruction of the $\Phi$ matrix inherit all this problems, returning a matrix with a  HSD far from expected. The question that arises is how this problems are solved. To answer it, we study how the TR behaves with the standard deviation $\sigma_E$ of each episode, which  are supposed to be the same.} The results are shown in Fig. \ref{fig:trace_simulation}(b). For $\sigma_E$ close to zero the distributions are all centered at $TR_e$ and the value of $\sigma_{TD}$ is reduced to 0.3 \gabo{(check)}. As  $\sigma_E$ increases, the center of the distribution of TR gets smaller values and its $\sigma_{TD}$ also increases. It is worth noting that the value of $\sigma_{TD}$ almost does not depends on the possible bettings $N$.  This explains why the distribution obtained in Fig. \ref{fig:trace_simulation} is not centered at the expected value.

%The time of convergence increases exponentially, causing long waiting times for larger data-sets, as observed in Fig. \ref{fig:trace_simulation}(d). This shows that our algorithm actually converges to the expected matrix when the simulated dataset has dimensions above $10^7$.      
%To make these magnitudes compatible with the theory, we extensively study the  problem of our algorithm in the presence of finite data. For this, lets suppose that in each of the 24 episodes the algorithm finds values that does not coincide with the expected maximum. Furthermore, lets consider that the algorithm converges values as far as possible from the expected. In this case, the reconstruction of the $\Phi$ matrix inherit all this problems, returning a matrix with a  TR far from expected. The question that arises is how this problems are solved. To answer it, we study how the TR behaves with the standard deviation $\sigma_E$ of each episode, which  are supposed to be the same. The results are shown in Fig. \ref{fig:trace_simulation}(b). For $\sigma_E$ close to zero the distributions are all centered at $TR_e$ and the value of $\sigma_{TD}$ is reduced to 0.3 \gabo{(check)}. As  $\sigma_E$ increases, the center of the distribution of TR gets smaller values and its $\sigma_{TD}$ also increases. It is worth noting that the value of $\sigma_{TD}$ almost does not depends on the possible bettings $N$.  This explains why the distribution obtained in Fig. \ref{fig:trace_simulation} is not centered at the expected value. Now, another question arises: how we physically  reduce the value of $\sigma_E$? The answer is in Fig. \ref{fig:trace_simulation}(c). We can see that as we increase $S$, $\sigma_E$ decreases, showing that the best  solution of the problem is obtained for larger $S$. However, this makes our convergence times exponencially larger as can be seen in Fig. \ref{fig:trace_simulation}(d). This shows that our algorithm actually converges to the expected matrix when the simulated dataset has dimensions above $10^7$.      

about the algorithm

%To obtain all the probabilities necessary to reconstruct the Eq. \ref{eq:vecBR}, we will need more than one hundreds episodes, causing an extremely long time of computation. For this reason, in what follows, we choose $N\approx 10^6$, reducing the time by a factor......


%The above description explains how we generated the data for our algorithm -- we next describe the algorithm itself. Each phase of the experiment is divided into `episodes' consisting of many `steps'. In each episode we designate an input state (one of either $\ketbra{\psi_s}{\psi_s}$ or $\ketbra{\pi_i}{\pi_i}$), detection angle $\Theta_m$, and a specific outcome (either $j \in {1,2}$ or $i \in {1,2,3,4}$) depending which phase of the experiment we are in). In each step, the algorithm must `bet' on the given outcome by choosing from a set of possible bets in the range $\{B_k = \frac{k}{N} : k=0,\dots,N \}$. After selecting its bets, the measurement is experimentally performed, and the agent receives a `reward' based on their bet and the outcome obtained. Over many steps, the agent adjusts their betting strategy according to a \tit{reinforcement learning} (RL) algorithm, until the `best' bet stabilizes at one of the $B_k$. This is then output as one of $B^{(1)}(j)$,$B^{(2)}(j|i)$,$B^{(2)}(i)$ depending on the episode and phase. 

%Our algorithm is based on a \tit{epsilon-greedy} algorithm. In our case, the reward function isto be the quadratic loss function described in the introduction. For example, suppose we are considering outcome $i=3$ and the agent chooses to bet $B_8$. If the detector corresponding to the outcome $i=3$ clicks in the $m$-th step, the agents `reward' for that step is $r_m(B_8) = -(\frac{8}{N}-1)^2$, otherwise they receive $r_m(B_8) = -(\frac{8}{N})^2$. The agent adds the rewards to a running total for each bet, i.e.\ after $M$ steps the total for bet $B_k$ is $T_k = \zum{m=1}{M} \, r_m(B_k)$. When deciding which bet to make, the epsilon-greedy algorithm has a $(1-\epsilon)$ chance of choosing the bet with the highest running total\footnote{If multiple bets share the same running total, it selects randomly among them} $B_{\trm{max}} := \{B_k : \trm{max}(T_k) \}$ and an $\epsilon$ chance of choosing any bet uniformly at random, with $\epsilon$ taken to be small. This algorithm thereby represents a conservative balance weighted in favour of `exploitation' (choosing bets that have been beneficial in the past) over `exploration' (taking a risk by trying other bets).

%Each phase of the experiment is divided into `episodes' consisting of many `steps'. In each episode we designate an input state (one of either $\ketbra{\psi_s}{\psi_s}$ or $\ketbra{\pi_i}{\pi_i}$), detection angle $\Theta_m$, and a specific outcome (either $j \in {1,2}$ or $i \in {1,2,3,4}$) depending which phase of the experiment we are in). In each step, the algorithm must `bet' on the given outcome by choosing from a set of possible bets in the range $\{B_k = \frac{k}{N} : k=0,\dots,N \}$. After selecting its bets, the measurement is experimentally performed, and the agent receives a `reward' based on their bet and the outcome obtained. Over many steps, the agent adjusts their betting strategy according to a \tit{reinforcement learning} (RL) algorithm, until the `best' bet stabilizes at one of the $B_k$. This is then output as one of $B^{(1)}(j)$,$B^{(2)}(j|i)$,$B^{(2)}(i)$ depending on the episode and phase. 



%For simplicity, we use a standard \tit{epsilon-greedy} algorithm, and define the reward function to be the quadratic loss function described in the introduction. For example, suppose we are considering outcome $i=3$ and the agent chooses to bet $B_8$. If the detector corresponding to the outcome $i=3$ clicks in the $m$-th step, the agents `reward' for that step is $r_m(B_8) = -(\frac{8}{N}-1)^2$, otherwise they receive $r_m(B_8) = -(\frac{8}{N})^2$. The agent adds the rewards to a running total for each bet, i.e.\ after $M$ steps the total for bet $B_k$ is $T_k = \zum{m=1}{M} \, r_m(B_k)$. When deciding which bet to make, the epsilon-greedy algorithm has a $(1-\epsilon)$ chance of choosing the bet with the highest running total\footnote{If multiple bets share the same running total, it selects randomly among them} $B_{\trm{max}} := \{B_k : \trm{max}(T_k) \}$ and an $\epsilon$ chance of choosing any bet uniformly at random, with $\epsilon$ taken to be small. This algorithm thereby represents a conservative balance weighted in favour of `exploitation' (choosing bets that have been beneficial in the past) over `exploration' (taking a risk by trying other bets).

miscellaneous

%\section{Experiment}
%\subsection{ RL Agent analysis}

%Due to the imprecision of our agent to learn probabilities from theoretical simulated data and the large amount of data required to learn the phi matrix, it is unclear whether our agent can learn the Phi matrix. Therefore, we test the agent's ability to learn the Phi matrix from data simulated from our experimental setup, specifically for the case of ideal states.

%For the simulation of each episode, we can think in the generation of a state of form $\alpha \ket{H}+\beta e^{i \varphi}\ket{V}$ where we choose $\varphi$ and $\alpha$  and one of the three bases to project:$\{H, V\}$,$\{D, A\}$, or $\{R, L\}$ randomly. Defined the states and the projection, we can calculate the $14$ probabilities needed for the episode. With these probabilities, we simulate data and feed the algorithm. After $24$ episodes, our agents find a Phi Matrix. As our agent presents fluctuations in the learning process, we learn $200$ different Phi matrices and use the trace distance of the phi matrix as a distance measurement. As is shown in Fig. \ref{fig:trace_simulation}, the trace of our Phi matrix is not centered on the theoretically expected value $10$ but is displaced. The averaged Phi matrix over the $200$ runs is

%To simulate each episode, we generate a state of the form $\alpha \ket{H}+\beta e^{i \varphi}\ket{V}$ with a randomly chosen projection from one of the three bases: $\{H, V\}$,$\{D, A\}$, or $\{R, L\}$. Using these states and projections, we calculate the $14$ required probabilities for the episode, simulate the data, and feed it to the algorithm. After $24$ episodes, our agents find a Phi Matrix, but due to fluctuations in the learning process, we learn 200 different Phi matrices and use the trace distance as a distance measurement. Fig. \ref{fig:trace_simulation} shows that the trace of our Phi matrix is displaced from the theoretically expected value of $10$. The averaged Phi matrix over the 200 runs is: 

%\begin{equation}
%\Phi=
 %   \begin{pmatrix}
   %     2.43 & -0.48& -0.47 & -0.44\\
     %   -0.48 & 2.44 & -0.46 & -0.49 \\
       % -0.49& -0.47 & 2.43 & -0.50 \\
        %-0.45 & -0.49 & -0.49 & 2.42
   % \end{pmatrix}
%\end{equation}



%To test if the problem is due to the fluctuation of the probabilities or if our agent is introducing another problem, we simulated data from the experiment but instead used our agent; we created a Gaussian distribution with different standard deviation and mean values around the probabilities calculated from our experiment to simulate our agent's imprecision and obtain the Figure \ref{fig:std}, showing that the shift in our trace is due to the imprecision of our agent and could be countered using a bigger data set.
%To determine if our agent's imprecision or probability fluctuations are responsible for the shift in the trace of our Phi matrix, we simulated data from the experiment but used our agent instead. We created a Gaussian distribution with various standard deviation and mean values around the experiment's calculated probabilities to simulate our agent's imprecision. The resulting Figure \ref{fig:std} shows that the shift in our trace is due to our agent's imprecision, which could be countered with a larger data set.







%First, we analyze the performance of our RL agent for different parameter values. We simulate data using a known probability distribution, feed the algorithm with it, and compare its output with its true value. Our agent gives us a different probability value for different runs, distributed as shown in Fig. \ref{fig:trace_dist}.  We can change three parameters in our algorithms: the number of discrete actions $A$, the number of steps $N$ (directly related to how much data our agent needs), and the $\epsilon$ value. It is worth mentioning the trade-off existing between the parameters: More steps and more actions lead to increase precision on the probabilities learned, but at the same time, increases the time and amount of data needed to converge, as is shown in fig \ref{fig:timeandstdvssteps}.
%For data process simulation, we can think in the throw of a biased coin with probability $p$, unknown for the agent but known to us. We feed our algorithm with different coin tosses, and after $N$ tosses (the number of steps), it returns the probability it thinks is best $p_{l}$, and we compare it with the known result $p$.
 %We choose for our agents the parameters $N=300000$, $\epsilon =0.5$, and $A=50$, for being the parameters that diminish the standard deviation (around 0.03) of our agent and give us a time that makes sense (around 12 hours of learning). 

%To analyze the performance of our RL agent, we simulated data using a known probability distribution and compared its output with the known probability $p$. An example of this comparison is shown in Fig. \ref{fig:trace_dist}. We changed three parameters in our algorithm: the number of discrete actions, the number of steps, and the epsilon value, which affected the precision of the probabilities learned and the time and amount of data needed to converge. We chose the parameters $N=300000$, $\epsilon=0.5$, and $A=50$, which reduced the standard deviation of our agent to around $0.03$ and took around 12 hours of learning, as we shown in Fig. \ref{fig:timeandstdvssteps}. We simulated the data by throwing a biased coin with probability $p$, unknown to the agent but known to us, and feeding the algorithm with different coin tosses. After N tosses, it returns the probability it thinks is best ($p_{l}$), which we compared with the known result ($p$).




%In fig \ref{fig:RF} we can observe how the reward functions learned for our agent change when we increase the number of steps. It is easy to understand the fluctuations of the learning process around the probability $p$ from this Figure. If the number of steps is insufficient to converge the reward function to the theoretical value, the maximum value could be confused with the fluctuations around the points.
%Fig. \ref{fig:RF} shows how the reward functions learned by our agent change as we increase the number of steps. The fluctuations in the learning process around the probability p can be easily observed from the figure. If the number of steps is not enough to converge the reward function to the theoretical value, the maximum value may be mistaken for the fluctuations around the points.



%Given the imprecision of our agent to learn the probabilities from theoretical simulated data and the vast quantity of data needed to learn the phi matrix, it is not a trivial question if our agent could learn the Phi matrix. That is why we test the agent's performance to learn the Phi Matrix from data simulated from our experimental setup for the case of ideal states.
%Due to the imprecision of our agent to learn probabilities from theoretical simulated data and the large amount of data required to learn the phi matrix, it is unclear whether our agent can learn the Phi matrix. Therefore, we test the agent's ability to learn the Phi matrix from data simulated from our experimental setup, specifically for the case of ideal states.


%For the simulation of each episode, we can think in the generation of a state of form $\alpha \ket{H}+\beta e^{i \varphi}\ket{V}$ where we choose $\varphi$ and $\alpha$  and one of the three bases to project:$\{H, V\}$,$\{D, A\}$, or $\{R, L\}$ randomly. Defined the states and the projection, we can calculate the $14$ probabilities needed for the episode. With these probabilities, we simulate data and feed the algorithm. After $24$ episodes, our agents find a Phi Matrix. As our agent presents fluctuations in the learning process, we learn $200$ different Phi matrices and use the trace distance of the phi matrix as a distance measurement. As is shown in Fig. \ref{fig:trace_simulation}, the trace of our Phi matrix is not centered on the theoretically expected value $10$ but is displaced. The averaged Phi matrix over the $200$ runs is

%To simulate each episode, we generate a state of the form $\alpha \ket{H}+\beta e^{i \varphi}\ket{V}$ with a randomly chosen projection from one of the three bases: $\{H, V\}$,$\{D, A\}$, or $\{R, L\}$. Using these states and projections, we calculate the $14$ required probabilities for the episode, simulate the data, and feed it to the algorithm. After $24$ episodes, our agents find a Phi Matrix, but due to fluctuations in the learning process, we learn 200 different Phi matrices and use the trace distance as a distance measurement. Fig. \ref{fig:trace_simulation} shows that the trace of our Phi matrix is displaced from the theoretically expected value of $10$. The averaged Phi matrix over the 200 runs is: 



%To test if the problem is due to the fluctuation of the probabilities or if our agent is introducing another problem, we simulated data from the experiment but instead used our agent; we created a Gaussian distribution with different standard deviation and mean values around the probabilities calculated from our experiment to simulate our agent's imprecision and obtain the Figure \ref{fig:std}, showing that the shift in our trace is due to the imprecision of our agent and could be countered using a bigger data set.
%To determine if our agent's imprecision or probability fluctuations are responsible for the shift in the trace of our Phi matrix, we simulated data from the experiment but used our agent instead. We created a Gaussian distribution with various standard deviation and mean values around the experiment's calculated probabilities to simulate our agent's imprecision. The resulting Figure \ref{fig:std} shows that the shift in our trace is due to our agent's imprecision, which could be countered with a larger data set.

experiment:

%The experimental outline runs as follows. An `agent' (implemented as an algorithm) receives the outcomes $i,j$ for the two alternative experiments depicted in  Fig.\ \ref{fig:Setup} as input data. In each run, the agent places `bets' by outputting numbers $B^{(1)}(j)$ for experiment One and $B^{(2)}(i),B^{(2)}(j|i)$ for experiment Two, for all values of $i,j$. The agent is then `rewarded' according to a pre-defined utility function that depends only on their choice of bet and the outcome obtained in the experiment (for simplicity we use the quadratic loss function mentioned in the Introduction). Depending on this feedback, the agent adjusts their betting behaviour in the next run according to some reinforcement-learning algorithm. This is repeated for all outcomes, holding $\rho, \mathcal{D}$ fixed, until the bets converge to approximately stable values; we take these bets to represent the algorithm's `posterior probabilities'\footnote{This interpretation is justified because -- insofar as it is reasonable to speak of the agent assigning probabilities at all -- the quadratic loss function ensures that the agent's probabilities must be numerically equal to its bets.} via the substitutions $B^{(1,2)} \leftrightarrow \trm{Pr}^{(1,2)}$ and use them to compute the components $q(j),\vec{r}(j),\vec{p}$ for this combination of $\rho, \mathcal{D}$, which will subsequently be analyzed for conformity to the Born rule. To make the results more robust, we perform this same process for a variety of different states and measurements. 


%\rodrigo{we must mention of the symetric hypotesis in the phi matrix used. we can explain sayinng that just measure states on the poles of Bloch Sphere and it were not enough, but with more states could be possible, as we show with simulate data... Or should we discuss that in the result section?}

%\subsection{RL agent using experimental data}
%Data were acquired for 10 minutes for each state and projection using the set-up in Figure (a) (20 for set-up b), divided into intervals of $5$ milliseconds, such that most of the time, only one coincidence was detected. Events with more than one coincidence or zero coincidences were discarded. For the entire experiment, we obtained a total of $24$ episodes ($6$ states x $4$ projections).

%Given that the amount of states obtained is insufficient to perform the linear regression, we reduced the number of variables to $10$, using the symmetry of the phi matrix as a hypothesis.

%To reach the number of steps necessary for acceptable convergence, we used the same experimental data set several times for learning each probability, mixing the data to avoid the appearance of patterns, and Finally obtaining the trace distribution showed in Fig. \ref{fig:trace_realdata} . The standard deviation and mean value agree with our theoretical model.

experimental details
% \subsection{Preliminaries: Naimark theorem}
%Given that in the lab all measurements performed are projective, the question of how POVM measurement are actually performed arises.   For this reason, the Naimark theorem plays an important role, providing recipe to obtain the POVM elements by coupling the system (polarization in our case) with an ancilla (spatial modes), and then performing projective measurements over it. Let us assume that the system and the ancilla are initially in the state $\ket{\Psi}_{SA}=\ket{\psi}_s\otimes \ket{\phi}_A$. The global evolution is given by a unitary operation, such that the evolved state is $U_{SA}\ket{\Psi}_{SA}$. Then, projective measurements are implemented on the ancilla in a orthogonal basis $\ket{b_i}$, where $i$ varies from 1 to 4. The probability of getting the result $i$ is given by
%\begin{equation}
%p_i=\textbf{Tr}_{S,A}\left[\left(\mathbb{I} \otimes \ket{b_i} \bra{b_i} \right)U_{SA}^{\dagger}\ket{\psi}_s\bra{\psi}\otimes \ket{\phi}_A\bra{\phi} U_{SA}\right].
%\end{equation}
% After reordering and taking a partial trace over the ancillary system leads to
%\begin{equation}
%p_i=\textbf{Tr}_{S}\left[ \mathbb{I}\cdot \textbf{Tr}_{A}\left(U_{SA}^{\dagger}\ket{b_i} \bra{b_i} U_{SA}\ket{\phi}_A\bra{\phi}\right) \\ \ket{\psi}_s\bra{\psi}\right],
%\end{equation}
%where  the identity operator is applied to the  polarization degree of freedom. For each value in $i$  the  POVMs can be  expressed as
%\begin{equation}
%\hat{\Pi}_i=\textbf{Tr}_{A}\left(U_{SA}^{\dagger}\ket{b_i} \bra{b_i}U_{SA} \ket{0}_A\bra{0}\right),
%\label{eq:POVMs}
%\end{equation}
%where we have made $\ket{\phi}=\ket{0} $

SIC implementation
%Based on the proposal in Ref. \cite{ling2006experimental}, the SIC-POVM measurement can be perfomed using a spatial  using the setup in Fig. \ref{fig:Setup}b). As can be seen from Eq. (\ref{eq:POVMs}), to obtain the POVMs it is necessary to have information of the global unitary operation $U_{SA}$.   For this, it is important to consider  the ancillary degrees of freedom required for the Naimark theorem, which correspond to the output propagation modes $b_i$. 

%Intermediate ancillary levels have also been considered to describe the modes propagation ($\ket{0}$, $\ket{1}$, $\ket{2}$ and $\ket{3}$) between the PPBS and the desplaced-Sagnac interferometer


convergence
%Consequently, this appendix substantiates our original hypothesis on the correlation between step size and accuracy of probability learning and extends its applicability to a wide array of probability values.


%As illustrated in Figure \ref{fig:differents_prob}, it is evident that the probability learned by our agent shifts based on the specific probability value we use. This observation led us to extend our results to a wider range of probability values. 


